Unified Generation, Reconstruction, and Representation: Generalized Diffusion with Adaptive Latent Encoding-Decoding

The vast applications of deep generative models are anchored in three core capabilities -- generating new instances, reconstructing inputs, and learning compact representations -- across various data types, such as discrete text/protein sequences and continuous images. Existing model families, like variational autoencoders (VAEs), generative adversarial networks (GANs), autoregressive models, and (latent) diffusion models, generally excel in specific capabilities and data types but fall short in others. We introduce Generalized Encoding-Decoding Diffusion Probabilistic Models (EDDPMs) which integrate the core capabilities for broad applicability and enhanced performance. EDDPMs generalize the Gaussian noising-denoising in standard diffusion by introducing parameterized encoding-decoding. Crucially, EDDPMs are compatible with the well-established diffusion model objective and training recipes, allowing effective learning of the encoder-decoder parameters jointly with diffusion. By choosing appropriate encoder/decoder (e.g., large language models), EDDPMs naturally apply to different data types. Extensive experiments on text, proteins, and images demonstrate the flexibility to handle diverse data and tasks and the strong improvement over various existing models.

==> tables/model_compare.tex <==
\begin{table}[h]
\begin{tabularx}{\textwidth}{c|CCC}
\hline
Methods   & Generation & Representation & Reconstruction \\ \hline
VAEs       &      \dmark     &      \cmark          &     \dmark     \\
GANs      &     \cmark       &        \xmark        &      \xmark      \\
Autoregressive model       &      \cmark     &      \xmark          &     \xmark     \\
Diffusion model&      \cmark      &        \xmark        &      \dmark      \\ 
Latent diffusion &      \cmark      &        \dmark        &      \dmark      \\ \hline
Ours      &    \cmark        &       \cmark         &        \cmark   \\
\hline
\end{tabularx}
\caption{The trilemma of deep generative models among generation, reconstruction, and presentation. \cmark: capable; \dmark: limited capable ; \xmark: incapable. }
\label{tab:model-compare}
\end{table}

==> tables/tasks.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{
\begin{tabular}{l|ccc}
\hline
Task         & Generation & Representation & Reconstruction \\ \hline\hline
Image manipulation                 &                            & \cmark                              & \cmark                              \\
Interpolation                      &                         & \cmark                              &       \cmark                             \\
Image Generation and Reconstruction\lgy{split in two rows}                        & \cmark                          &                                    &   \cmark                               \\ \hline
Text Generation and Reconstruction & \cmark                          &                                    & \cmark                              \\
Style transferring                 &                                & \cmark                              & \cmark                              \\
Sentence interpolation             &              \cmark                & \cmark                              &  \cmark                                  \\ \hline
Protein representation             &                                & \cmark                              &                                    \\
Protein optimization               & \cmark                          &                \cmark                  & \cmark                              \\ \hline
\end{tabular}
}
\label{tab:tasks}
\caption{A summary of tasks and required ability for generative model.}
\end{table}

==> tables/text_interpolation.tex <==
\begin{table}[ht]
% \renewcommand{\arraystretch}{0.99}
    \centering
    \footnotesize
    \vspace{-19pt}
    \begin{tabular}{l|l}
    \toprule
Input-1&i ca n't believe how inconsiderate this pharmacy is .\\
Input-2&we were sat right away and every staff member was extremely friendly and happy .\\\midrule
\multirow{12}{*}{VAE}&i ca n't believe how inconsiderate this pharmacy is .\\
&i was n't so worried about how pharmacy membership is an inconvenience .\\
&i was n't worried about how inconsiderate this pharmacy is .\\
&i was n't asked how inconsiderate this pharmacy is .\\
&i was n't asked how trustworthy this pharmacy is .\\
&i was shocked how inconsiderate this pharmacy is .\\
&i was shocked ... how inconsiderate this pharmacy is .\\
&i was shocked ... how inconsiderate this staff is extremely friendly .\\
&i was sent ... how inconsiderately friendly and extremely disappointed .\\
&we were sat right away and every staff member was extremely friendly and accommodating .\\
&we were sat right away and every staff member was extremely friendly and welcoming .\\
&we were sat right away and every staff member was extremely friendly and happy .\\ \midrule
\multirow{20}{*}{DAAE}&i ca n't believe how inconsiderate this pharmacy is .\\
&i ca n't believe how very inconsiderate this pharmacy is .\\
&i ca n't believe how very inconsiderate this store is .\\
&i could n't believe how very inconsiderate this store is .\\
&i could n't believe how very inconvenient this restaurant is .\\
&i could n't believe how very indifferent this pharmacy staff is .\\
&i could not say how very inconvenient this store was friendly .\\
&i could not say how very inconvenient the staff is being and i am very disappointed .\\
&i could not say how very inconvenient the staff was being and i am very disappointed .\\
&i could not say how very inconvenient the staff was being so friendly .\\
&i could not say how very inconvenient the staff was extremely friendly and welcoming .\\
&i could not say very much about the locker owner and was very welcomed .\\
&i could not sit down and every friend was charging it was very uncomfortable .\\
&we were so rudely referred to every good gas company and was extremely rude .\\
&we were so rudely sat at every friend and it was extremely friendly .\\
&we were sat down and every friend and staff was extremely happy .\\
&we were sat down very much and the staff member was extremely friendly and welcoming .\\
&we were sat right away and every staff member was extremely happy .\\
&we were sat right away and every staff member was extremely friendly and welcoming .\\
&we were sat right away and every staff member was extremely friendly and happy .\\ \midrule
\multirow{12}{*}{\modelname}&i ca n't believe how inconsiderate this pharmacy is .\\
&i ca n't believe how inconsiderate this staff is .\\
&i 'm not sure how this pharmacy is .\\
&i 'm not impressed how inconsiderate this place is .\\
&i am very impressed and every customer service is great .\\
&i was very impressed and every customer service was great .\\
&i was very impressed and every staff member was amazing .\\
&we were very impressed and every staff member was extremely friendly .\\
&we were very impressed and every staff member was extremely friendly and helpful .\\
&we were very impressed ... every staff member was extremely friendly and helpful .\\
&we were sat right away and every staff member was extremely friendly and helpful .\\
&we were sat right away and every staff member was extremely friendly and happy .\\
\bottomrule
    \end{tabular}
    \vspace{-7pt}
    \caption{Examples of sentence interpolation with 50 steps. To avoid redundancy, repetitive outputs from adjacent steps are omitted.}
    \label{tb:exmaple_text_interpolation1}
\end{table}

\begin{table}[ht]
% \renewcommand{\arraystretch}{0.99}
    \centering
    \small
    \vspace{-19pt}
    \begin{tabular}{l|l}
    \toprule
Input-1&she was not happy being there .\\
Input-2&the chips and guacamole were excellent too !\\\midrule
\multirow{6}{*}{VAE}&she was not happy being there .\\
&the chips were cheap too .\\
&the chips were cheap and definitely excellent .\\
&the chips were cheap and excellent !\\
&the chips and guacamole were excellent !\\
&the chips and guacamole were excellent too !\\\midrule
\multirow{10}{*}{DAAE}&she was not happy being there .\\
&she was not happy with the food being there .\\
&she was not happy with the food and was not there .\\
&she was so happy and had fun being there .\\
&she was so happy and the food was excellent too .\\
&they were so happy with the food and it was delicious !\\
&the food was sooooo delicious and i was happy to have found it .\\
&the food was sooooo delicious and i was happy to have found it !\\
&the food was sooooo delicious and i was very happy !\\
&the chips and guacamole were excellent too !\\ \midrule
\multirow{7}{*}{\modelname}&she was not happy being there .\\
&she was not happy .\\
&she was not happy !\\
&she was happy !\\
&the food was excellent !\\
&the chips and salsa were excellent too !\\
&the chips and guacamole were excellent too !\\
\bottomrule
    \end{tabular}
    \vspace{-7pt}
    \caption{Examples of sentence interpolation with 50 steps. To avoid redundancy, repetitive outputs from adjacent steps are omitted.}
    \label{tb:exmaple_text_interpolation2}
\end{table}
